The B2Scala Tool: Integrating Bach in Scala with Security in Mind

Process algebras have been widely used to verify security protocols in a formal manner. However they mostly focus on synchronous communication based on the exchange of messages. We present an alternative approach relying on asynchronous communication obtained through information available on a shared space. More precisely this paper first proposes an embedding in Scala of a Linda-like language, called Bach. It consists of a Domain Specific Language, internal to Scala, that allows us to experiment programs developed in Bach while benefiting from the Scala eco-system, in particular from its type system as well as program fragments developed in Scala. Moreover, we introduce a logic that allows to restrict the executions of programs to those meeting logic formulae. Our work is illustrated on the Needham-Schroeder security protocol, for which we manage to automatically rediscover the man-in-the-middle attack first put in evidence by G. Lowe.

==> eptcsdata.tex <==
\providecommand{\firstpage}{58}
\providecommand{\publicationstatus}{C. Aubert, C. Di Giusto, S. Fowler \& V. K. I Pun (Eds.):\\
17th Interaction and Concurrency Experience (ICE 2024)\\
EPTCS 414, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.414.4}{10.4204/EPTCS.414.4}}
\pdfoutput=1

